Pix2Evidence: A Multimodal RAG System for Text and Visual Evidence

Retrieval-augmented generation (RAG) over visually rich documents must find both relevant content and the evidence that supports an answer. Screenshot retrieval preserves images and page structure, but written facts within screenshots also need to be searchable. Moreover, topical relevance alone does not identify which retrieved tile contains evidence for the answer. We introduce Pix2Evidence, a multimodal RAG system that encodes each screenshot tile together with its available transcription into a single fused image--text representation, so that layout and readable text are considered jointly during retrieval. To guide evidence selection, a vision-language teacher describes the visible content that supports each training question. We use these descriptions to adapt the retriever, then rerank the retrieved candidates before answer generation. Extensive experiments demonstrate that Pix2Evidence outperforms state-of-the-art methods. Across five widely-used Wikipedia QA benchmarks, the non-reranked Pix2Evidence leads the main comparison in answer accuracy on four. On MMSearch, it reaches 26.0\%, 4.4 percentage points above PixelRAG. We will release the code and share derived data where licensing and privacy reviews permit.

==> table_style.tex <==
% =====================================================================
% Grouped-header booktabs style (as used for the PixelRAG main table)
%
% Required in the preamble:
%   \usepackage{booktabs}   % \toprule \midrule \bottomrule \cmidrule
%   \usepackage{array}      % only if you use >{...} column specifiers
%
% Works in one column; use the starred form (\begin{table*}) when the
% table must span both ACL columns. The \cmidrule(lr) trim is what
% separates adjacent benchmark groups, so do not drop the (lr).
% =====================================================================


% ---------------------------------------------------------------------
% 1. Reference: the table exactly as it appears in the screenshot
% ---------------------------------------------------------------------
\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
& \multicolumn{2}{c}{NQ} & \multicolumn{2}{c}{NQ-Tables} & \multicolumn{2}{c}{SimpleQA} & \multicolumn{2}{c}{MMSearch} & \multicolumn{2}{c}{EVQA} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
Method & Recall & Acc & Recall & Acc & Recall & Acc & Recall & Acc & Recall & Acc \\
\midrule
No retrieval & \multicolumn{2}{c}{30.4} & \multicolumn{2}{c}{24.5} & \multicolumn{2}{c}{7.0} & \multicolumn{2}{c}{12.7} & \multicolumn{2}{c}{27.2} \\
\midrule
\multicolumn{11}{@{}l}{\textit{Text-based retrieval}} \\
\quad mwparserfromhell & 48.6 & 54.2 & 34.8 & 35.9 & 74.2 & 60.7 & -- & 25.3 & 6.5 & 31.5 \\
\quad Trafilatura & 45.8 & 55.9 & 37.2 & 42.5 & 77.4 & 71.6 & -- & 24.7 & 6.4 & 29.6 \\
\midrule
\multicolumn{11}{@{}l}{\textit{Pixel-based retrieval}} \\
\quad PIXELRAG (base) & 53.5 & 57.9 & 45.5 & 47.0 & 80.8 & 73.8 & -- & \textbf{28.3} & 27.1 & 40.7 \\
\quad PIXELRAG & \textbf{58.8} & \textbf{58.7} & \textbf{51.1} & \textbf{48.8} & \textbf{83.8} & \textbf{78.8} & -- & 28.3 & \textbf{35.0} & \textbf{45.1} \\
\bottomrule
\end{tabular}
\caption{Main results. Recall is evidence recall; Acc is answer accuracy
 judged by an LLM. A dash marks a metric that is not defined for that
 benchmark. Bold marks the best value in a column.}
\label{tab:pixelrag-style}
\end{table*}


% ---------------------------------------------------------------------
% 2. Blank skeleton of the same style
%    Replace the placeholder rows. For G groups of 2 metrics each the
%    column spec is @{}l + 2G copies of c, and the header spans are
%    \multicolumn{2}{c}{...} with \cmidrule(lr){start-end} underneath.
% ---------------------------------------------------------------------
% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% & \multicolumn{2}{c}{Benchmark A} & \multicolumn{2}{c}{Benchmark B} & \multicolumn{2}{c}{Benchmark C} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
% Method & Recall & Acc & Recall & Acc & Recall & Acc \\
% \midrule
% Baseline & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{7}{@{}l}{\textit{Group heading}} \\
% \quad Variant one & -- & -- & -- & -- & -- & -- \\
% \quad Variant two & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{7}{@{}l}{\textit{Group heading}} \\
% \quad Our method & -- & -- & -- & -- & -- & -- \\
% \bottomrule
% \end{tabular}
% \caption{Caption above the table, per ACL style.}
% \label{tab:skeleton}
% \end{table*}


% ---------------------------------------------------------------------
% 3. Same style applied to the current PixelsEvidence main results
%    Values are the verified ones already used in the paper, kept as
%    three-decimal fractions. Multiply by 100 for one-decimal
%    percentages if you prefer the unit used in section 1.
%    SimpleQA and MMSearch are single-metric groups, so their header
%    spans one column each and the sub-header row leaves those cells
%    empty.
% ---------------------------------------------------------------------
\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}lcccccc@{}}
\toprule
& \multicolumn{2}{c}{NQ} & \multicolumn{2}{c}{NQ-Tables} & \multicolumn{1}{c}{SimpleQA} & \multicolumn{1}{c}{MMSearch} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
Retriever & EM & Judged & EM & Judged & & \\
\midrule
\multicolumn{7}{@{}l}{\textit{Encoder A, image-only}} \\
\quad without reranking & 0.306 & 0.594 & 0.258 & 0.470 & 0.728 & 0.207 \\
\quad with reranking & 0.305 & 0.603 & 0.265 & 0.482 & 0.734 & 0.237 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Encoder B, image-only}} \\
\quad without reranking & 0.301 & 0.580 & 0.256 & 0.461 & 0.676 & 0.203 \\
\quad with reranking & 0.301 & 0.577 & 0.256 & 0.459 & 0.677 & 0.197 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Encoder B, fused, single branch}} \\
\quad without reranking & 0.321 & 0.602 & 0.257 & 0.469 & 0.723 & 0.243 \\
\quad with reranking & 0.319 & 0.600 & 0.257 & 0.469 & 0.724 & \textbf{0.250} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Encoder B, fused union text, two branches}} \\
\quad with reranking & \textbf{0.327} & \textbf{0.627} & \textbf{0.273} & \textbf{0.501} & \textbf{0.785} & 0.243 \\
\bottomrule
\end{tabular}
\caption{Recorded Wikipedia results. A and B denote different trained
 encoders, so rows describe system configurations rather than a
 controlled alignment comparison. Scores are fractions and bold marks
 the largest reported value in a column. The two-branch row without
 reranking is not available.}
\label{tab:main-restyled}
\end{table*}


% ---------------------------------------------------------------------
% 4. Alignment ablation, paper version (main.tex, Table 4).
%    Caption above the tabular, as in the PixelRAG Table 4 screenshot.
%    The three-value column layout (name / alignment / weight) plus a
%    final QA column is what the run records support.
% ---------------------------------------------------------------------
\begin{table}[t]
\centering
\small
\caption{Recorded evidence-alignment variants on the 400-question SimpleQA
 development subset, together with the alignment-free reference recorded
 for the same retriever recipe. QA is the peak value over training
 checkpoints; the six alignment runs stop at steps 100, 100, 100, 200,
 100 and 150 in table order. Weight is the coefficient of
 $\mathcal{L}_{\mathrm{align}}$ in Eq.~\ref{eq:loss}, and ``description''
 denotes a cosine penalty between the question and the description
 embeddings. Direction, weight and stopping step vary together across the
 rows, so the table records configurations and does not isolate the
 contribution of the alignment term.}
\label{tab:align-style}
\begin{tabular}{@{}lccc@{}}
\toprule
Run & Alignment & Weight & QA \\
\midrule
contrastive only & -- & -- & 0.7725 \\
\textbf{fwdKL\_kl0005} & \textbf{forward KL} & \textbf{0.05} & \textbf{0.7900} \\
fwdKL\_kl02 & forward KL & 0.20 & 0.7825 \\
revKL\_kl02 & reverse KL & 0.20 & 0.7800 \\
descalign\_w01 & description & 0.10 & 0.7750 \\
realignREV\_kl005 & reverse KL & 0.05 & 0.7750 \\
descalign\_w02 & description & 0.20 & 0.7725 \\
\bottomrule
\end{tabular}
\end{table}


% ---------------------------------------------------------------------
% 5. Optional wider variant: keep the peak retrieval score and the step
%    at which each run peaked. Use this one if a reviewer asks whether
%    the rows were stopped at the same point; the peak steps differ, and
%    the contrastive-only row has no recorded step.
% ---------------------------------------------------------------------
% \begin{table}[t]
% \centering
% \small
% \caption{Same runs as Table~\ref{tab:align-style}, with the peak
% Recall@1 and the step at which each run peaked.}
% \label{tab:align-wide}
% \begin{tabular}{@{}lcccrc@{}}
% \toprule
% Run & Alignment & Weight & R@1 & Step & QA \\
% \midrule
% contrastive only & -- & -- & 0.7625 & -- & 0.7725 \\
% fwdKL\_kl0005 & forward KL & 0.05 & 0.7675 & 100 & \textbf{0.7900} \\
% fwdKL\_kl02 & forward KL & 0.20 & 0.7650 & 100 & 0.7825 \\
% revKL\_kl02 & reverse KL & 0.20 & 0.7600 & 100 & 0.7800 \\
% descalign\_w01 & description & 0.10 & 0.7600 & 200 & 0.7750 \\
% realignREV\_kl005 & reverse KL & 0.05 & 0.7600 & 100 & 0.7750 \\
% descalign\_w02 & description & 0.20 & 0.7625 & 150 & 0.7725 \\
% \bottomrule
% \end{tabular}
% \end{table}

